Dynamic distributed decision-making for resilient resource reallocation in disrupted manufacturing systems

The COVID-19 pandemic brings many unexpected disruptions, such as frequently shifting markets and limited human workforce, to manufacturers. To stay competitive, flexible and real-time manufacturing decision-making strategies are needed to deal with such highly dynamic manufacturing environments. One essential problem is dynamic resource allocation to complete production tasks, especially when a resource disruption (e.g., machine breakdown) occurs. Though multi-agent methods have been proposed to solve the problem in a flexible and agile manner, the agent internal decision-making process and resource uncertainties have rarely been studied. This work introduces a model-based resource agent (RA) architecture that enables effective agent coordination and dynamic agent decision-making. Based on the RA architecture, a rescheduling strategy that incorporates risk assessment via a clustering agent coordination strategy is also proposed. A simulation-based case study is implemented to demonstrate dynamic rescheduling using the proposed multi-agent framework. The results show that the proposed method reduces the computational efforts while losing some throughput optimality compared to the centralized method. Furthermore, the case study illustrates that incorporating risk assessment into rescheduling decision-making improves the throughput.

==> sections/5_4_complexity.tex <==
\subsection{Complexity analysis}
\label{sec:comlexity}

\rev{In this section, we analyze how the proposed method reduces the problem complexity.
Based on the schedule definition, time constraints, and risk assessment in this work, the scheduling problem is similar to a job shop scheduling problem, which is NP-hard.
Therefore, re-generating the total schedule in a centralized way to deal with disruption requires large computational efforts.
The proposed method uses agent communication as a heuristic to find a solution (instead of the optimal solution) to the job shop rescheduling problem following three steps: (1) identify the minimal changes needed to the initial schedule, (2) find candidate new schedule via agent local coordination, and (3) determine the new schedule that optimizes the user-defined objectives.}

\rev{In (1), the disrupted agent $RA_d$ evaluates its event schedule $s(RA_d)$ to identify the affected events $E_d$, whose time complexity is $O(|s(RA_d)|)$ at the worst case (i.e., all the events are affected).
Each affected event $e_{d_i}$ corresponds to a PA $PA_{d_i}$, then the PA needs to identify the minimal changes needed to the schedule.
This time complexity is $O(|s(RA_d)|\times \max{|s(PA_{d_i})|)}$ at the worst case (i.e., all the schedules need to be changed).}

\rev{In (2), the disrupted agent $RA_d$ evaluates the clustering agents for each affected event $e_{d_i}$.
This process takes $O(|E_d|\times\max{|C_{\ell}(e_{d_i},RA_d)|})$ at the worst case.
However, as mentioned in Section~\ref{sec:racoord}, the clustering agents may propagate the communication if needed.
Denote $Z_{j}$ as the set of agents that one clustering agent $RA_j$ propagates the communication to, then we have the time complexity $O(|E_d|\times\max{|C_{\ell}(e_{d_i},RA_d)|})\times \max|Z_j|$).
The complexity grows as the agents propagate communication.
Therefore, we set several constraints, such as resource attributes and a limited number of schedule shifts, to stop the communication, which may give no schedule as discussed in Section~\ref{sec:decisionmaking}.}

\rev{In (3), determining the new schedule from the candidate set $S_{new}$ could be a naive sorting problem to find the minimal completion time.
One common algorithm for this problem takes $O(|S_{new}|)$ to compute.}

\rev{In conclusion, the proposed method is a heuristic method to find several feasible candidate new schedules via agent communication, then determine the new schedule based on user-defined objectives.
Therefore, the complexity of each step is lower than solving the job shop rescheduling problem in one step.
However, the optimality of the solution highly depends on agent communication, and it is sub-optimal in most cases.
From the system level, it is not difficult to verify the new schedule is a solution but it is still not verifiable in polynomial time that the new schedule is an optimal solution.
}
